UTFix: Change Aware Unit Test Repairing using LLM

Software updates, including bug repair and feature additions, are frequent in modern applications but they often leave test suites outdated, resulting in undetected bugs and increased chances of system failures. A recent study by Meta revealed that 14%-22% of software failures stem from outdated tests that fail to reflect changes in the codebase. This highlights the need to keep tests in sync with code changes to ensure software reliability. In this paper, we present UTFix, a novel approach for repairing unit tests when their corresponding focal methods undergo changes. UTFix addresses two critical issues: assertion failure and reduced code coverage caused by changes in the focal method. Our approach leverages language models to repair unit tests by providing contextual information such as static code slices, dynamic code slices, and failure messages. We evaluate UTFix on our generated synthetic benchmarks (Tool-Bench), and real-world benchmarks. Tool- Bench includes diverse changes from popular open-source Python GitHub projects, where UTFix successfully repaired 89.2% of assertion failures and achieved 100% code coverage for 96 tests out of 369 tests. On the real-world benchmarks, UTFix repairs 60% of assertion failures while achieving 100% code coverage for 19 out of 30 unit tests. To the best of our knowledge, this is the first comprehensive study focused on unit test in evolving Python projects. Our contributions include the development of UTFix, the creation of Tool-Bench and real-world benchmarks, and the demonstration of the effectiveness of LLM-based methods in addressing unit test failures due to software evolution.

==> figure/changed_diff.tex <==
\begin{center}
    \begin{minipage}{0.9\textwidth}
        \small
        \begin{lstlisting}[escapeinside={(*@}{@*)},style=Python-github]
def create_table(self, name: str, fields: Sequence[Dict[str, Any]], description: Optional[str]=None) -> 'pyairtable.api.table.Table':
  url = self.meta_url(""tables"")
- payload = {"name": name, "fields": fields}
+ payload = {'name': name + ""_modified"", 'fields': fields[:1]}
  if description:
-   payload["description"] = description
+   payload["description"] = description[:10] #Truncated
  response = self.api.post(url, json=payload)
- return self.table(response[""id""], validate=True, force=True)
+ return self.table(response['id'], validate=False, force=False)
        \end{lstlisting}
    \end{minipage}
    \captionof{figure}{\change{}d Diff}
    \label{fig:technique_diff_fm}
\end{center}


==> figure/feedback_prompt.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.9\textwidth}
        \begin{tcolorbox}[colback=white, colframe=white, boxsep=0pt, top=0pt, bottom=0pt, left=0pt, right=0pt]
            \begin{lstlisting}[escapeinside={(*@}{@*)},style=Python-github]
For more information, following two types of program context are provided:
<optional_focal_method_context>
    <static_context>  {slice_for_context}  </static_context>
    <dynamic_context> {dynamic_trace}   </dynamic_context>
</optional_focal_method_context>
            \end{lstlisting}
        \end{tcolorbox}
    \end{minipage}
    \caption{An example of static and dynamic context provided in the program}
    \label{fig:static_context}
\end{figure}


==> response.tex <==
\clearpage

\section{Response Letter}
\label{sec:response}
We thank the reviewers for their valuable questions and comments. In this section, we provide details for how we address all questions and  comments. We first respond to the metareview comments and then respond
to each reviewer by dividing each reviewer's concerns into (1)~Questions from ``Questions for authors’ response'', (2)~Questions
from ``Detailed comments for authors'', and (3)~Comments from ``Detailed comments for authors''.
Note that in our revised draft with tracking, we highlight only the substantial changes made to address questions and comments from reviewers to avoid excessive color that could obscure the main revisions.
We discuss and refer to the highlighted changes in this response
letter.
%Note that, in our revised draft, we highlight only the substantial changes made to address reviewer comments—avoiding excessive color that could obscure the main revisions. These highlighted changes are discussed in this response letter.

% Note that in our revised draft with tracking, we do not highlight every change we made from
% our initial submission to avoid having the paper be filled mainly with colors, thereby making it more difficult to read the substantial changes.
% Instead, we highlight only the substantial changes we made to address questions and comments from reviewers. We discuss and refer to the highlighted changes in this response letter.

\Comment{Detailed review
META-REVIEW: (This is only a meta-review, so please ignore the scores given above.)

Thank you for your submission to OOPSLA 2025. Overall, the reviewers appreciate the authors' responses to their questions and hope the authors can address the following points in a major revision:

    1. Extensively use open-source models in the evaluation. e.g., Codellama or DeepSeek-Coder.
    2. Address the data leakage problem in the discussion section.
    3. Add a strong argument about the real-world significance of critical assertion failures and reduced code coverage caused by focal method changes.
    4. Add experiments or clearly explain why the generated dataset is not biased toward the proposed approach.
    5. Consider more sophisticated alternative methods for matching the primary focal method with its corresponding unit test.
    6. Add more background knowledge or details to improve the presentation of the motivating example.
    7. Other revisions promised in the response.
}
\subsection{Metareview Comments}
\subsubsection{Extensively use open-source models in the evaluation.} %\Fix{@Baishakhi}
\label{ques:metareview1}
\begin{itemize}
    \item We conducted experiments using \opensource{} models from \huggingface{}~\cite{huggingface} following the same experimental setup as of \Tool{}. This includes the same structured prompts with the same content across four prompt settings-no context (\toolNASym{}), static context (\toolSSym{}), dynamic context (\toolDSym{}), and a combination of static and dynamic context (\toolSDSym{})- as well as \COT{} using five times feedback. 

    
    \begin{itemize}
        \item \llama{} Evaluation:
        \begin{itemize}[label=$\blacksquare$]
            %\item We used \codellamaThirteenBIntruct{}   but observed poor performance, with only \codellamaAF{}\%  of tests repaired.
            %\item We use the latest version of the \llama{} family models, specifically the \llamaThreeB{}. Our findings indicate that it successfully repairs \llamaThreeBAF{} of tests with \af{}, compared to a baseline (i.e., \llamaThreeB{} with the changed \fm{}) repair rate of \llamaThreeBBaselineAF{}. Additionally, to enhance \cc{}, \llamaThreeB{} achieves 100\% \cc{} in \llamaThreeBCC{} tests, compared to the baseline of \llamaThreeBaselineBCC{} tests.
           \item We use the latest version of the \llama{} family models, specifically the \llamaThreeB{}. Our findings indicate that \llamaThreeB{} with \toolDSym{} achieves the highest \af{} repair rate among all prompt settings, \llamaThreeBAF{} of tests, compared to a baseline (i.e., \llamaThreeB{} with the changed \fm{}) repair rate of \llamaThreeBBaselineAF{}. Additionally, to improve \cc{}, \llamaThreeB{} with \toolSSym{} is the most effective, achieving 100\% \cc{} in \llamaThreeBCC{} tests, compared to the baseline of \llamaThreeBaselineBCC{} tests.
        \end{itemize}
        \item \deepSeekCoder{} Evaluation:
            \begin{itemize}[label=$\blacksquare$]
                \item We conducted experiments with \deepSeekCoder{} and found that \deepSeekCoderVInstruct{} requires substantial GPU resources, needing at least 8 GPUs with 80GiB each for the generation task as it is a 236B MoE model. Due to this limitation, we use \deepSeekCoderVLite{} which is less resource-intensive and has 16B total parameters with 2.4B active parameters.
                
            \item Using 2.4B active parameter \deepSeekCoderVLite{} with \toolDSym{}, we achieve the highest \af{} repair rate among all prompt settings,  \deepSeekCoderVLiteAF{}, compared to a baseline repair rate of \deepSeekCoderVLiteBaselineAF{}. Furthermore, to improve \cc{}, \deepSeekCoderVLite{} with \toolSSym{} is the most effective, achieving 100\% \cc{} in \deepSeekCoderVLiteCC{} tests, compared to the baseline of \deepSeekCoderVLiteBaselineCC{} tests.                 
            \end{itemize}
    \end{itemize}
    %Across both models, we find that for \af{}, \toolDSym{} achieves the highest repair rate, while \toolSSym{} is the most effective  in improving \cc{}, which aligns with the \Tool{}'s findings. 
     We have added this description to Section~\ref{sec:discussion}: ``
                We conducted experiments using \opensource{} models...''.
    %\Shanto{use the same text from section 7}
\end{itemize}


\subsubsection{Address the data leakage problem in the discussion section.}
\label{ques:metareview2}
\begin{itemize}
    \item %To prevent data leakage, \Tool{} is mainly evaluated on uniquely changed \fm{}s generated in-house, ensuring they are new, distinct, and not publicly available. Still, as our subject projects are collected from open-source GitHub repositories, we validate the uniqueness of the changed \fm{}s by randomly sampling \Num{20} examples from five projects and thoroughly reviewing their commit histories using keyword searches and manual verification. No matches were found in the commit history that corresponded to our dataset, minimizing the risk of overlap with any data seen during the training of LLMs like \sonnet{}. 
    To prevent data leakage, \Tool{} is primarily evaluated on uniquely changed \fm{}s generated in-house, ensuring they are new, distinct, and not publicly available. Since our subject projects are collected from \opensource{} \github{} repositories, we validate the uniqueness of the changed \fm{}s by randomly sampling \Num{20} examples from five projects and thoroughly reviewing their commit histories using keyword searches and manual verification. No exact matches of the \fm{} diffs were found in prior commits, meaning that the specific code changes used in our dataset have not appeared before. This minimizes the risk of overlap with any data seen during the training of LLMs like \sonnet{}. \Comment{\Fix{Further, given the baseline and our method have been evaluated on the same model on the same date, in the presence of potential data leakage, our method still demonstrates improvements over baseline.}} We have added this explanation to Section~\ref{sec:discussion}: ``\Tool{} is primarily evaluated on uniquely changed...''.

    %\Shanto{Does the fix exist in real data? If not, also you can mention that. Further, you can say that }
\end{itemize}
\subsubsection{Add a strong argument about the real-world significance of critical assertion failures and reduced code coverage caused by focal method changes.}
\label{ques:metareview3}
\begin{itemize}   

    \item %\Shanto{Why do not you add this line here from Intro?}  
    Meta’s study shows that 14\%-22\% of failures come from outdated test cases that do not reflect changes in the codebase~\cite{vahabzadeh2015empirical}.

    \item Software testing and reliability literature identify \af{} and insufficient test coverage as key factors affecting reliability~\cite{daniel2009reassert, wang2024hits, avdeenko2021automated, khemka2024toward}. Repairing these issues in evolving software is crucial, as ignoring or deleting failing tests compromises the test suite’s effectiveness~\cite{daniel2009reassert}. Moreover, a recent study by Microsoft revealed that test cases are the most important area where developers need help from AI tools~\cite{khemka2024toward}. These findings underscore the importance of addressing \af{} and reduced \cc{} to ensure robust and reliable software. We have added this discussion in Section~\ref{sec:intro}: ``Software testing and reliability literature identify...''.
    
    \item In our experiments, we collected \realExample{} \realWorld{} instances from \realExampleProjects{} heavily used \github{} projects, \curated{} from their main branches, showing \af{} and reduced \cc{} as the \fm{} evolved (described in Section~\ref{sec:curate-real-changes}). The presence of such un-updated \utest{}s in the main branch highlights the critical need for repairing them. 
\end{itemize}


\subsubsection{Add experiments or clearly explain why the generated dataset is not biased toward the proposed approach.}
\label{ques:metareview4-dataset-bias}

\begin{itemize}
    \item Our \benchmark{} encompasses \NumDifferentChanges{} different types of \fm{} changes—including API modifications, concurrency issues, error-handling adjustments, and more—that lead to \af{} and low \cc{}. This diversity ensures that the dataset reflects various \realWorld{} challenges rather than being tailored to a specific approach. Moreover, \Tool{} does not rely on any assumptions about the type of change; it simply focuses on the location of changes and the nature of the resulting errors to repair \utest{}. This design choice guarantees that our dataset is unbiased and representative of a broad spectrum of issues encountered in practice.
    We have added this explanation in Section~\ref{sec-diversity-rq4}: ``Our \benchmark{} encompasses...''.

    \item To assess potential bias, we also sample \realWorld{} data and apply \Tool{} directly to demonstrate its effectiveness in \realWorld{} scenarios where \af{} and reduced \cc{} occur. This validation on developer-written data, rather than synthetically generated examples, ensures that \Tool{} generalizes beyond curated datasets and mitigates concerns about potential bias.
\end{itemize}


\subsubsection{Consider more sophisticated alternative methods for matching the primary focal method with its corresponding unit test.}
\label{ques:metareview5}
\begin{itemize} 
    \item %\Shanto{read} 
    The main rationale behind our \fm{} and \utest{} matching is that the \utest{} should execute the \fm{}. However, in complex \realWorld{} scenarios, a \utest{} often includes setup calls before invoking the primary \fm{}. For example, Figure~\ref{fig:expected_values} shows a case where Lines ~\ref{line:setupCallOneInTest} and \ref{line:setupCallTwoInTest} contain setup calls before the actual \fm{} call at Line~\ref{line:actualMethodCallInTest}. Therefore, we inject changes into the \fm{}. To focus on the main functionality, we choose a heuristic that selects the method with the closest name similarity to the \fm{} among all methods executed by the \utest{}.
    We further ensure that the \fm{} is indeed executed when the \utest{} runs, as evidenced by the call graph or execution traces (described in Section~\ref{sec:find_test_fm_pairs_by_running_test}). To address potential concerns that name similarity could introduce bias in the repair process, we conducted an additional experiment where we replaced the test name in a \utest{} using a combination of random string generation and regex-based substitution. We then applied \Tool{} to determine whether the \utest{} could still be repaired. Our results indicate that \Tool{} successfully repaired 99.34\% of the tests compared to the original repair rate and achieved 100\% \cc{} for 96 tests, the same as the original repair. We have added this description in Section~\ref{sec:threats}: ``However, we ensure that the \fm{} is indeed executed...''. 
    
\Comment{\begin{itemize}
    \item We generate a new test name by replacing the existing  name in a \utest{} using a combination of random string generation and regex-based substitution.
    \item Then we apply \Tool{} to see if the \utest{} can be repaired.
    \item Our results show that \Tool{} can repair  99.34\%\Comment{(303/305} of the test compared to the original repair rate.
    \item Our results show that \Tool{} can achieve 100\% \cc{} for 96 tests, which is exactly the same number as the original repair.   
\end{itemize}}
\end{itemize}


\subsubsection{Add more background knowledge or details to improve the presentation of the motivating example.}
\begin{itemize}
    \item We have added background knowledge in the Related Work Section~\ref{sec:related}: ``The application of \LLM{}s... TestART generates unit test...''.  
    \item We have explained more clearly the motivating examples at Section~\ref{sec:example}. 
    \item In Figure~\ref{fig:example-af}, we have added the definition of the \CodeIn{reloaded} variable at Line~\ref{line:definitionOfReloadedVar}.  
\end{itemize}

\subsubsection{Other revisions promised in the response.}
\begin{itemize}
    \item We promised to share the code and data. 
    \begin{itemize}
        \item Our scripts and data are available~\cite{SitesUTFixCodeAndScript}. We have added this in Section~\ref{sec:dataAvailable}: ``Our artifact is available...''.
    \end{itemize}
    %\item \Fix{What else ...}
\end{itemize}

\subsection{Reviewer A}
\MyParaColon{Questions from ``Detailed comments for authors''}

 \begin{enumerate}
   \item Missing Citations:  
   - TOGA: A Neural Method for Test Oracle... (ICSE 2022), Using pre-trained language models... (ISSTA 2022), TestART: Improving LLM-based Unit Test...

   \begin{itemize}
    \item We have added these citations along with their descriptions in Section~\ref{sec:related}: ``The application of LLMs... TestART generates unit test...''.
   \end{itemize}
 \item Figure 10 needs more explanation:
    * Why does including both traces seem to yield worse results than using either the static or dynamic method alone?
    \begin{itemize}
    \label{ques:why_dynamic_trace_works_better_than_combined}
        \item We have included an explanation in Figure~\ref{fig:test-repair-subfigures}: ``Both figures show that...''.
        \item Combining both static and dynamic traces (i.e., contexts) sometimes yields worse results because these contexts together provide conflicting or redundant information, which can confuse the model. We have added a more detailed description in Section~\ref{sec:eval-rq1}: ``Static context includes...''. 
    \end{itemize}
 \item Discussion on unfixed tests:
    * The paper lacks insights into tests that remain unfixed. Would combining traditional methods with LLMs yield better outcomes?
    \label{quesA:unfixed-bug}
   \begin{itemize}
        \item \Tool{} restricts test repair to within the body of the test code. So, \Tool{} fails to \repair{} tests if the \repair{} falls outside the test code. This may happen for parameterized tests where expected values are defined externally or tests reliant on external setups, such as mock objects. Expanding \Tool{}’s repair scope to handle these external setups could address such issues. Furthermore, certain \repair{}s may fall outside the scope of automated solutions, particularly when the specifications of the underlying \fm{} are unknown or cannot be inferred. In such cases, involving a human in the loop will be essential. We have added this explanation in Section~\ref{sec:threats}: ``\Tool{} restricts test repair...''. 
   \end{itemize}
\item On model selection:
    * UTFix only used Claude 3.5 Sonnet. Were any open-source models used or compared? Additionally, computational resource requirements and energy efficiency considerations are not addressed.
   \begin{itemize}
        \item We have addressed this question in Metareview Comments ~\ref{ques:metareview1}. 
        \item We have discussed the computational resource requirements and energy efficieny in Section~\ref{sec:setup-running-env}: ``We run our experiments using...''. 
   \end{itemize}
\item Language support:
    * Is UTFix limited to Python, or can it be adapted to support other programming languages?

    \begin{itemize}
        \item \Tool{} is currently implemented for Python, as our dataset is based on Python projects. However, the core principles and methodology of \Tool{} are language-agnostic, focusing on analyzing and repairing tests and their corresponding \fm{}s. With appropriate datasets and adaptations for language-specific syntax and testing frameworks, \Tool{} can be extended to support other programming languages. 
        This discussion is added in Section~\ref{sec:threats}: ``The core principles and methodology...''.
    \end{itemize}

\item Data leakage concerns: * UTFix used an LLM. Were measures taken to prevent any data leakage, considering that some tasks for open-source projects may have been seen by Claude 3.5 Sonnet during training?
\begin{itemize}
    \item We have addressed this in Metareview Comments~\ref{ques:metareview2}.
\end{itemize}
 \end{enumerate}

\subsection{Reviewer B}
\MyParaColon{Questions from ``Questions for authors’ response''}
 \begin{enumerate}
  \item How to ensure the quality of the curated datasets?
  \begin{itemize}
    \item Assessing the quality of AI-generated data remains an open challenge, though research highlights that careful prompting can significantly enhance data quality~\cite{liu2024refining}. Building on this approach, we ensure quality across four dimensions:
    \begin{itemize}
        \item Syntactic and Semantic correctness: All \curated{} changes are verified as compilable by running tests.
        \item Realistic Development Scenario: For \benchmark{} with reduced \cc{}, we verify that tests pass while achieving less than 100\% coverage, reflecting realistic scenarios of incomplete testing. 
        \item Diversity: We prioritize varied \fm{} changes, including `error handling', `API updates', `branches', `loops', and `data structure' changes.
        \item Manual Checking: Additionally, we conducted a manual spot check on a subset of the data to ensure its quality (e.g., obvious hallucination is not present, etc.). 
    \end{itemize}
    
We have added this discussion in Section~\ref{sec:eval_dataset}: ``Assessing the quality of AI-generated...''.
  \end{itemize}

  \item How to collect code-coverage?
   \begin{itemize}
     \item 
     To collect \cc{}, we instrument \CodeIn{tox.ini} (an automated tool primarily used in Python to run tests) with \CodeIn{pytest-cov} to track executed lines. We then run tests in isolation via tox, generating a coverage report. Since this report only lists covered line numbers without specifying executed \fm{} lines, we analyze the \fm{}'s \AST{} and intersect it with the report to extract \cc{}.
     We have updated the text in Section~\ref{sec:context-collection}: ``To collect \cc{}...''.
   \end{itemize}

   \item Do we need to repair all the assertion failures?
   \begin{itemize}
   \item In \realWorld{} software evolution, both the \fm{} and the associated \utest{} can be incorrect. However, \Tool{} operates in a regression setting, assuming that the \fm{} has been correctly evolved. Our evaluation data is \curated{} based on this assumption, and the experiments are conducted accordingly. Thus, ideally, \Tool{} should \repair{} all the \af{} as such failures usually reflect the actual behavior and the expected value differ, highlighting potential bugs or unsatisfied requirements. Since we are assuming the \fm{} is correct, the bugs are thus coming from the \utest{}. We have added this discussion in Section~\ref{sec:discussion}: ``In real-world software evolution...''.
     \end{itemize}

   \item When would UTFix fail to fix, and how can this problem be addressed?
   \begin{itemize}
   \item Please see the answer to Questions from ``Detailed comments for authors''~\ref{quesA:unfixed-bug} (Reviewer A). \Tool{} restricts test repair to within the test body, failing when fixes require external setups like parameterized tests or mock objects. Expanding its scope could address such cases. Additionally, some repairs remain infeasible without known \fm{} specifications, necessitating human involvement. 
   \end{itemize}
\end{enumerate}


\MyParaColon{Questions from ``Detailed comments for authors''}
\begin{enumerate}
    \item Clarity: Some examples and explanations are difficult to follow, leading to confusion. Additional questions:
        \begin{enumerate}[label=(\roman*)]
            \item What is the definition of `reloaded' in the first motivating example?
            \begin{itemize}
                \item The definition of \CodeIn{reloaded} is as follows and has been added to Figure~\ref{fig:exampleRepairedTestAF} at Line~\ref{line:definitionOfReloadedVar}.\\
                    reloaded = api.bases(force=True)
                \item The \CodeIn{reloaded} object contains all base IDs from bases except one specific ID ('appSW9R5uCNmRmfl6'), as \CodeIn{force=True}. This is because the \fm{} excludes this ID when \CodeIn{force=True} in Figure~\ref{fig:exampleFocalMethodAF} at Lines~\ref{line:exampleFMAddedLineAFa}-\ref{line:exampleFMAddedLineAF}.
                Retaining the original assertion (Lines~\ref{line:exampleTestDeletedLineAFa}-\ref{line:exampleTestDeletedLineAF}) then leads to an \af{} since \CodeIn{reloaded} no longer matches \CodeIn{base\_ids}. Hence, in the repaired test, the assertion is updated to explicitly check the first base ID in reloaded (reloaded[0].id) against the expected value `appLkND'.  We have updated the details in Section~\ref{sec:example-assertion-fail}: ``The changed \fm{}...''.
                \end{itemize}
            \item How does the updated code provide a more straightforward way...?
            \begin{itemize}
                %\item In the second example, the repaired test makes a direct call to delete\_api at Lines~\ref{line:exampleResultFMAddedLinea}-\ref{line:exampleResultFMAddedLine}, reducing the abstraction in the test code. A mock object is already configured to return an HTTP status code of 200 that indicates a successful at Line~\ref{line:exampleTestMockReturnSuccess}. Following this setup, after finishing the for loop, the test verifies that the mock DELETE request was called the expected number of times  at Lines~\ref{line:exampleTestAssertionLinea}-\ref{line:exampleTestAssertionLine}, based on how the input data (ids) is chunked and processed at Line~\ref{line:exampleTestUpdateForLoopCC}. We add the details into the revised text of the paper.
                
            \item 
            %In Figure~\ref{fig:exampleFocalMethod}, the \fm{} \CodeIn{batch\_delete} has been changed to handle empty inputs. A new condition is introduced to check if the \CodeIn{record\_ids} list is empty (Line~\ref{line:exampleResultFMAddedConditionLine}). If the input is empty, the \fm{} immediately returns an empty list without making unnecessary API calls, ensuring optimal performance at Line~\ref{line:exampleResultFMReturnedLineCC}. In Figure~\ref{fig:exampleRepairedTest}, the corresponding test \CodeIn{test\_batch\_delete} is updated to reflect the changes in the \fm{} and ensure full  \cc{}. Specifically, a new assertion is added to verify the behavior for empty input (\CodeIn{batch\_delete([])}), ensuring that the \fm{} returns an empty list as expected at Line~\ref{line:exampleNewAssertionForCC}.  This ensure that the updated test achieves 100\% \cc{}, covering all possible execution paths, including the new empty input condition. 
            In Figure~\ref{fig:exampleFocalMethod}, the \fm{} \CodeIn{batch\_delete} is modified to handle empty inputs by returning an empty list (Line~\ref{line:exampleResultFMReturnedLineCC}) instead of making unnecessary API calls.  The updated test \CodeIn{test\_batch\_delete} (Figure~\ref{fig:exampleRepairedTest}) adds a new assertion (Line~\ref{line:exampleNewAssertionForCC}) verifies that \CodeIn{batch\_delete([])} returns an empty list, while the original assertion (Line~\ref{line:exampleOrigAssertionForCC}) still validates non-empty inputs. This ensures 100\% \cc{} by covering all execution paths. We have updated the text in Section~\ref{sec:example-reduced-cc}: `` A new assertion...''.

%for \CodeIn{batch\_delete([])}, ensuring full \cc{}, including the new empty input condition (Line~\ref{line:exampleNewAssertionForCC}). We have updated the text in Section~\ref{sec:example-reduced-cc}:  ``A new condition is introduced to check if...''.

%A new assertion (Line~\ref{line:exampleNewAssertionForCC}) verifies that \CodeIn{batch\_delete([])} returns an empty list}, while the original assertion (Line~\ref{line:exampleOrigAssertionForCC}) still validates non-empty inputs. \Mr{This ensures 100\% \cc{} by covering all execution paths}.

            \end{itemize}
            
            \item Additionally, the paper did not mention how UTFix might lead to false positives. It would be helpful to include examples of these false positives and an analysis explaining why UTFix fails to address them.
            \begin{itemize}
                \item  In \Tool{}, a `false positive' repair might be considered if a test is updated and marked as repaired without truly repairing the error. To ensure repair reliability, we run each test \Num{10} times, confirming consistent passing results. Additionally, we manually review a sample of \Num{10} repairs to verify their effectiveness and confirm no `false positives', ensuring \Tool{} genuinely addresses the issues in the original tests. We have added this discussion in Section~\ref{sec:discussion}: ``In \Tool{}, a ‘false positive’ repair...''.  
            \end{itemize}
        \end{enumerate}
    
        \item Is the Data-Availability Statement reasonable?
    \begin{itemize}
        \item Our script and data are available at this link~\cite{SitesUTFixCodeAndScript}.
    \end{itemize}
\end{enumerate}

\MyParaColon{Comments from ``Detailed comments for authors''}

\begin{enumerate}
    \item  I also expect the authors to justify the choice of evaluation metrics and discuss limitations associated with them.
    \begin{itemize}
        \item In our evaluation of \Tool{}, we prioritize metrics that directly assess its effectiveness in repairing tests impacted by changes in the \fm{}. Specifically, we focus on resolving \af{} and improving \cc{}, as these are critical indicators of a successful test repair. While other metrics, such as mutation scores, could provide additional insights, we believe that concentrating on these primary factors offers a more accurate assessment of \Tool{}'s performance in a differential testing context. This approach ensures that our evaluation aligns with the core objective of verifying \Tool{}'s capability to address immediate test failures resulting from code changes. By focusing on \af{} and improved \cc{}, we aim to provide a clear and practical evaluation of \Tool{}'s effectiveness. We have added this discussion in Section~\ref{sec:threats}: ``While other metrics, such as mutation...''.
    \end{itemize}
\end{enumerate}

\subsection{Reviewer C}
\MyParaColon{Questions from ``Questions for authors’ response''}
\begin{enumerate}
  \item Can you provide evidence demonstrating how critical assertion failures and reduced code coverage caused by focal method changes are in real-world scenarios?
  \begin{itemize}
  %\label{ques:how_critical_issues_are_we_handling}
  \item Please see the answer to Metareview Comment~\ref{ques:metareview3}.
  \end{itemize}

  \item Why were other alternative methods for matching the primary focal method with the corresponding unit test not considered?
   \begin{itemize}
    \label{ques:other_alternative_approaches}
     \item We have addressed this in Metareview Comment~\ref{ques:metareview5}.
   \end{itemize}
\end{enumerate}

\MyParaColon{Questions from ``Detailed comments for authors''}
\begin{enumerate}
    \item The authors focus on repairing unit test cases... However, it is unclear how critical these two issues are in practice. The authors should conduct a study to demonstrate that these are indeed the primary challenges encountered during focal method evolution.
    \begin{itemize}
        \item We have addressed this in Metareview Comment~\ref{ques:metareview3}.
    \end{itemize}

    \item The proposed methodology for addressing the problem and generating the dataset appears relatively straightforward, relying primarily on prompting large language models. Consequently, the work feels more like an engineering effort than a significant research contribution. \Comment{\Fix{Not added anywhere in the paper yet. In fact, I am not sure if we need to add it into anywhere in the paper.}}
    \begin{itemize}
        \item Our key contribution is a systematic approach to repair \utest{} during code evolution, addressing issues such as \af{} and low \cc{}. \Tool{} modifies or adds assertions, updates test prefixes, and dynamically adapts tests to reflect changes in the \fm{}. It leverages static and dynamic analyses, combined with an iterative feedback loop using an LLM, to repair \utest{}s based on real-time execution feedback. Additionally, \Tool{} includes an execution validator to automate validation, ensuring repaired tests are syntactically and semantically correct, and achieving high reliability and coverage, as demonstrated in Figure~\ref{fig:utgFramework} of our paper. We believe this approach advances automated test repair beyond traditional engineering practices.
        While substantial engineering efforts were necessary, our primary innovation is incorporating static and dynamic slices w.r.t. the \fm{} changes directly into the prompting context and further improve the performance with guided feedback. 
    \end{itemize}
    \item In the dataset generation process, the authors determine the primary focal method for a given unit test solely based on the similarity between their names. However, other alternative approaches might have done a better job, such as call graph analysis, execution trace matching, and dependency analysis. Incorporating these strategies could improve the generalizability and reliability of the dataset.

    \begin{itemize}
        \item Please see the answer to Metareview Comment~\ref{ques:metareview5}.
    \end{itemize}

\item The dataset seems to be designed specifically to address the two issues emphasized by the authors, which may introduce bias in evaluating repaired unit tests. Certainly, there could be other potential scenarios for repairing unit tests, such as handling API changes, issues related to concurrency, error handling, and so on.
 \begin{itemize}
        \item We have addressed this in Metareview Comment~\ref{ques:metareview4-dataset-bias}.
    \end{itemize}

    
    \item  In the evaluation results, it is surprising that the dynamic approach outperforms the combined static and dynamic approach. The authors should investigate this further to understand the underlying reasons behind this outcome.
    
    \begin{itemize}
        \item Please see the answer to Questions from ``Detailed comments for authors' response (Reviewer A)''~\ref{ques:why_dynamic_trace_works_better_than_combined}.  
    \end{itemize}    

    \item Is the Data-Availability Statement reasonable? It looks to me all the codes used in the benchmark generation come from Github. What legal restrictions apply to the availability of the data?
    \begin{itemize}
      \item  Our script and data are available at this link~\cite{SitesUTFixCodeAndScript}.
    \end{itemize}    
    %\item * there could be other potential scenarios for repairing unit tests, such as handling API changes … *
\end{enumerate}
    
%\MyParaColon{Comments from ``Detailed comments for authors''}

%\begin{enumerate}
%    \item it is 
%    \begin{itemize}
%       \item Yes. 
%    \end{itemize}
%\end{enumerate}

==> tables/diversity_changes_for_rq4.tex <==
\input{figure/assertion_modification.tex}

\begin{table}[h]
    \centering
    \begin{minipage}{\textwidth} % Using minipage instead of tabular
        \centering
        \input{figure/assertion_modification} % Include the figure content
        \textbf{(a) Assertion Modification} \\[10pt]
    \end{minipage}
    \caption{Figures arranged in rows: (a) Assertion Modification, (b) Expected Values, (c) Branch Coverage.}
    \label{fig:figures_in_table}
\end{table}


==> technique.tex <==
% \section{Our \Tool{}}
% \label{sec:technique}

%\include{technique-benchmark}
%\include{technique-repair}

% Base Prompt Box
\tcbset{
    baseprompt/.style={colback=blue!5!white, colframe=blue!50!black, fonttitle=\bfseries}
}
\Comment{
\begin{figure}[h]
    \centering
    \begin{minipage}{\textwidth}
        \begin{tcolorbox}[title=Base Prompt, colback=white, colframe=white, boxsep=0pt, top=0pt, bottom=0pt, left=0pt, right=0pt]
            \noindent\rule{\textwidth}{0.4pt}  % Top horizontal line
            \begin{verbatim}
<instructions>
    You are analyzing a software testing situation. A unit 
    test case that previously passed is now failing due to 
    an update in the *focal method* it was testing. You have 
    the following information:
    1. The failing unit test case is provided in the 
    `<unit_test>` tag.
    2. The error message or failure output from the test is 
    given in the `<failure_message>` tag.
    3. The changed focal method is given in the 
    `<changed_focal_method>` tag.
    Your task is to:
    1. Repair the test method, ensuring it covers the 
    changes made in the focal method. 
        a. Wrap your repaired test in 
        `<repaired_test_method>` tag.
        b. Mention the changes you made using 
        `<modification_type>` tag.
        c. Ensure the entire response, 
        `<repaired_test_method>` and `<modification_type>` 
        tags are wrapped in a `<root>` tag to maintain 
        well-formed XML.
    2. Follow the constraints provided under the 
    `<constraints>` tag while fixing/updating the test.
</instructions>
<constraints>
    The repaired test must pass.
</constraints>

<data>
    <diff_focal_method> {diff_fm_code} </diff_focal_method>
    <unit_test> {unit_test_body} </unit_test>
    <failure_message> {failure_message}  </failure_message>  
</data>
            \end{verbatim}
            \noindent\rule{\textwidth}{0.4pt}  % Bottom horizontal line
        \end{tcolorbox}
    \end{minipage}
    \caption{Base prompt structure for analyzing a software testing situation}
    \label{fig:base_prompt}
\end{figure} }



\Comment{
In this heuristics, we extract the changes that happened in the focal method. We also extract the failure message when running the tests. Finally, we also include the faulty unit test to repair the test. 
\subsubsection{\DiffPlusStaticSlice{} of focal method}
2. Used Static Trace
\subsubsection{\DiffPlusDynamicTrace{} of focal method}
3. Used Dynamic Trace


\subsection{Unit Test Generation}
\label{sec:generationtechnique}
Unlike the \test{} \repair{}, here our goal is to improve \cc{}, 
1. Used only diff of focal method, unit test and test failure message
2. Used Dynamic Trace
3. Used Static Trace}





